A Compositional Approach to Safety-Critical Resilient Control for Systems with Coupled Dynamics

Complex, interconnected Cyber-physical Systems (CPS) are increasingly common in applications including smart grids and transportation. Ensuring safety of interconnected systems whose dynamics are coupled is challenging because the effects of faults and attacks in one sub-system can propagate to other sub-systems and lead to safety violations. In this paper, we study the problem of safety-critical control for CPS with coupled dynamics when some sub-systems are subject to failure or attack. We first propose resilient-safety indices (RSIs) for the faulty or compromised sub-systems that bound the worst-case impacts of faulty or compromised sub-systems on a set of specified safety constraints. By incorporating the RSIs, we provide a sufficient condition for the synthesis of control policies in each failure- and attack- free sub-systems. The synthesized control policies compensate for the impacts of the faulty or compromised sub-systems to guarantee safety. We formulate sum-of-square optimization programs to compute the RSIs and the safety-ensuring control policies. We present a case study that applies our proposed approach on the temperature regulation of three coupled rooms. The case study demonstrates that control policies obtained using our algorithm guarantee system's safety constraints.

==> feasibility.tex <==
\section{Verifying the Feasibility of Indices and Control Policies}

The optimization problem in Eqn. \eqref{eq:QP} is solved in real time and the control inputs given by Eqn. \eqref{eq:QP} ensures that the system is safe. However, Eqn. \eqref{eq:QP} may not always be feasible. In this section, we verify the feasibility of constraint \eqref{eq:QP 1} in an offline manner.

Our idea is to find the largest set $\tilde{\mathcal{C}}_k\subseteq\mathcal{C}_k$ so that constraint \eqref{eq:QP 1} is feasible for the corresponding $\gamma_i^k$ and $\beta$. We define $\tilde{\mathcal{C}}_k=\{x\in\mathcal{C}_k:h_k(x)\geq c_k\}$ with $c_k\geq 0$. In this case, we compute $\gamma_i^k$ as follows:
\begin{subequations}\label{eq:gamma constrained}
\begin{align}
    \min_{\gamma_i^k}~ &-\gamma_i^k\\
    \st ~&\frac{\partial h_k}{\partial x_i}(f_{ii}(x_i)+g_{ii}(x_i)u_i)\nonumber\\
    &\quad\quad\quad-\gamma_i-p_1(x)(h_k(x)-c_k)-q_1(x,u_i)v(u_i)\geq 0
\end{align}
\end{subequations}
where $p_1(x)$ and $q_1(x,u_i)$ are SOS polynomials. Note that this optimization problem is non-convex when $\tilde{\mathcal{C}}_k$ is unknown. Similarly, the value of $\beta$ can be obtained as:
\begin{subequations}\label{eq:beta constrained}
\begin{align}
    \min_{\beta^k}~ &-\beta^k\\
    \st ~&\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})u_i)\nonumber\\
    &-\beta^k-p_2(x)(h_k(x)-c)-\sum_{i=m+1}^Nq_{i,2}(x,u_i)v_i(u_i)\geq 0
\end{align}
\end{subequations}

Given the values of $\gamma_i^k$ and $\beta^k$, the feasibility of constraint \eqref{eq:QP 1} over set $\tilde{\mathcal{C}}_k$ can be computed by verifying if the following expression is an SOS or not:
\begin{multline}\label{eq:feasibility SOS}
    \frac{\partial h_k}{\partial x_i}[f_{ii}(x_i)+g_{ii}(x_i)\mu_i(x) + f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})\mu_i(x)]\\
    - \alpha_i\left(-\eta_i(h_k(x))-\beta^k-\sum_{j=m+1}^N\gamma_j^k\right)
    -\lambda(x)(h_k(x)-c),
\end{multline}
where $\lambda(x)$ is an SOS polynomial and $\mu_i(x)$ is a polynomial in $x$. We formally state this result as follows.
\begin{proposition}
Given $\gamma_i^k$ for each $i\in\{m+1,\ldots,N\}$ and $\beta^k$, if the expression in Eqn. \eqref{eq:feasibility SOS} is an SOS, where $\lambda(x)$ is an SOS polynomial and $\mu_i(x)$ is a polynomial in $x$, then constraint \eqref{eq:QP 1} is feasible for all $x\in\tilde{\mathcal{C}}_k$ when $u_i$ is chosen as $u_i=\mu_i(x)$.
\end{proposition}
\begin{proof}
Since $\lambda(x)$ is an SOS polynomial, we have that $\lambda(x)(h_k(x)-c)\geq 0$ for all $x\in\tilde{\mathcal{C}}_k$. When Eqn. \eqref{eq:feasibility SOS} is an SOS, we thus have that 
\begin{multline*}
    \frac{\partial h_k}{\partial x_i}[f_{ii}(x_i)+g_{ii}(x_i)\mu_i(x) + f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})\mu_i(x)]\\
    - \alpha_i\left(-K_i(h(x))-\beta^k-\sum_{j=m+1}^N\gamma_j^k\right)\geq 0
\end{multline*}
holds for all $x\in \tilde{\mathcal{C}}_k$. When $u_i=\mu_i(x)$, we have that constraint \eqref{eq:QP 1} is feasible over $\tilde{\mathcal{C}}_k$.
\end{proof}

In the following, we mitigate the non-convexity introduced due to the construction of set $\tilde{\mathcal{C}}_k$. We propose Algorithm \ref{algo:C1} to compute the value of $c_k$, $\gamma_i^k$, $\beta^k$, and verify the feasibility of constraint \eqref{eq:QP 1} simultaneously. We remark that Algorithm \ref{algo:C1} can be implemented in an offline manner, and it terminates within $\lceil \frac{\Bar{c}_k}{\epsilon}\rceil$ iterations in the worst-case, where $\Bar{c}=\sup_{x\in\mathcal{C}_k}h_k(x)$ and $\epsilon$ is the step size that can be tuned.

\begin{center}
  	\begin{algorithm}[!htp]
  		\caption{Solution algorithm for guaranteeing the feasibility of constraint \eqref{eq:QP 1}.}
  		\label{algo:C1}
  		\begin{algorithmic}[1]
  			\State \textbf{Input}: Dynamics $F$. Functions $h_k$ and $v_i$. Parameter $\epsilon>0$
  			\State \textbf{Output:} Parameters $\{\gamma_i^k\}_{i=m+1}^N$, $\beta^k$, and $c_k$
  			\State \textbf{Initialization}: Initialize $\Bar{c}_k\leftarrow\sup_{x\in\mathcal{C}_k}h_k(x)$, $c_k\leftarrow0$, $Flag\leftarrow 0$
            \While{$Flag = 0$ and $c_k\leq \Bar{c}_k$}
            \State Solve the SOS programs in Eqn. \eqref{eq:gamma constrained} and \eqref{eq:beta constrained} to calculate $\gamma_i^k$ for each $i\in\{m+1,\ldots,N\}$ and $\beta^k$\label{line:gamma beta}
            \State Verify if Eqn. \eqref{eq:feasibility SOS} is an SOS or not using $\gamma_i^k$ and $\beta^k$ obtained from line \label{line:gamma beta}
            \If{Eqn. \eqref{eq:feasibility SOS} is an SOS}
            \State $Flag\leftarrow 1$
            \Else 
            \State $c_k\leftarrow c_k+\epsilon$
            \EndIf
            \EndWhile\label{line:iter end}
            \State \textbf{return} $c_k$, $\{\gamma_i^k\}_{i=m+1}^N$, and $\beta^k$
  		\end{algorithmic}
  	\end{algorithm}
  \end{center}

==> formulation.tex <==
\section{System Model and Problem Formulation}\label{sec:formulation}

This section presents the system model and our problem formulation.

We consider a system $\mathcal{S}$ consisting of a finite set of interconnected sub-systems, denoted as $\{\mathcal{S}_i\}_{i=1}^N$. For each sub-system $\mathcal{S}_i$, it follows dynamics:
\begin{align}
    \mathcal{S}_i:\dot{x}_i=&f_{i, self}(x_i)+g_{i,self}(x_i) u_i\nonumber\\
    &+f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i
\end{align}
where $x_i\in\mathbb{R}^{n_i}$ is the state of sub-system $\mathcal{S}_i$, $x_{-i}\in\mathbb{R}^{n-n_i}$ is the state of other sub-systems excluding $\mathcal{S}_i$, $u_i\in\mathbb{R}^{r_i}$ is the input, $f_{i, self}:\mathbb{R}^{n_i}\rightarrow\mathbb{R}^{n_i}$, $g_{i,self}:\mathbb{R}^{n_i}\rightarrow\mathbb{R}^{n_i\times r_i}$,  $f_{i,coupled}:\mathbb{R}^{n_i}\times\mathbb{R}^{n-n_i} \rightarrow\mathbb{R}^{n_i}$, and $g_{i,coupled}:\mathbb{R}^{n_i}\times \mathbb{R}^{n-n_i}\rightarrow\mathbb{R}^{n_i\times r_i}$. We assume that $f_{i, self},g_{i,self},f_{i,coupled},g_{i,coupled}$ are Lipschitz. Here functions $f_{i, self}$ and $g_{i,self}$ are dependent on the states of sub-system $\mathcal{S}_i$ only. We refer the dynamics corresponding to $\Big(f_{i, self}(x_i)+g_{i,self}(x_i) u_i\Big)$ as \textit{self-dynamics} of sub-system $\mathcal{S}_i$. On the other hand functions $f_{i,coupled}$ and $g_{i,coupled}$ are jointly determined by the states of $x_i$ and those of other sub-systems $x_{-i}$. We refer the dynamics corresponding to $\Big(f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i\Big)$ as  \textit{coupled-dynamics} of sub-system $\mathcal{S}_i$. 

Let $x=[x_1^T ~\cdots~x_N^T]^T\in\mathbb{R}^n$ and $u=[u_1^T~\cdots~u_N^T]^T\in\mathbb{R}^r$ where $n=\sum_{i=1}^Nn_i$ and $r=\sum_{i=1}^Nr_i$. Then the dynamics of $\mathcal{S}$ can be written as
\begin{equation}\label{eq:joint dynamics}
    \mathcal{S}:\begin{bmatrix}\dot{x}_1\\
    \vdots\\
    \dot{x}_N
    \end{bmatrix}=\begin{bmatrix}
    F_1(x_1,x_{-1},u_1)\\
    \vdots\\
    F_N(x_N,x_{-N},u_N)
    \end{bmatrix}\triangleq F(x,u)
\end{equation}
where $F_i(x_i,x_{-i},u_i)=f_{i, self}(x_i)+g_{i,self}(x_i) u_i +f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i$.

We consider that system $\mathcal{S}$ is given $K$ safety constraints for all time $t\geq 0$ where $K \in \mathbb{Z}_{+}$. We suppose each safety constraint is represented as $h^k(x) \geq 0$ where $h^k:\mathbb{R}^n\rightarrow \mathbb{R}$ is a continuously differentiable function for each $k=1,\ldots,K$. We denote the corresponding safety set as $\mathcal{C}$ so that $\mathcal{C}=\cap_{k=1}^N \{x\in \mathbb{R}^n: h^k(x) \geq 0\}$.

Some sub-system $\mathcal{S}_i$ is subject to random failures and malicious attack. In these scenarios, the actuator of sub-system $\mathcal{S}_i$ does not behave as expected. In the following, we assume that there exists a subset of sub-systems such that they are protected and does not incur random failures or attack. We denote this set of sub-systems as $\mathcal{N}_1=\{1,\ldots,m\}$ and refer them as \textit{protected sub-systems}. In addition, the set of sub-systems that can incur random failures or compromised by the adversary is denoted as $\mathcal{N}_2=\{m+1,\ldots,N\}$ and we refer them as \textit{vulnerable sub-systems}.

In this paper we are interested in finding control policies in the protected sub-systems which will ensure safety of system $\mathcal{S}$ irrespective of the conditions of the vulnerable subsystem. We state the problem of interest as follows:
\begin{problem} \label{prob1}
Consider system $\mathcal{S}$ where only a subset of sub-systems $\mathcal{N}_2$ is subject to random failures and malicious attacks. Compute a control input $u_i$ for each $i \in \mathcal{N}_1$ at each time $t$ such that system $\mathcal{S}$ is safe with respect to $\mathcal{C}$. 
\end{problem}

==> introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Cyber-physical systems (CPS) are vulnerable to random failures and cyber-attacks which can potentially cause damage to the system and even endanger human lives. Therefore CPS especially critical infrastructure are required to maintain safety even under failures or attacks.
Cyber-physical Systems (CPS) \cite{ames2016control,cohen2020approximate,fan2020fast} have been shown to be vulnerable to random failures and cyber-attacks, which can cause safety violations. Safety violations of CPS can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. Therefore, safe operation of CPS under fault or attack has become a priority, especially for critical infrastructure.


To this end, defense against attacks, fault-tolerant design and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, safety analysis and control of safety-critical CPS become challenging as the complexity and scale of CPS increase. Specifically, CPS with multiple interconnected sub-systems may have multiple distinct safety requirements. In addition, as more sub-systems are interconnected, the system dimension increases, making some existing approaches designed for low-dimensional system intractable. Furthermore, an intelligent adversary can utilize additional surfaces to attack the system as more sub-systems are interconnected. A comprehensive protection against attack over entire system may be impractical for large-scale CPS.


% Many of efforts for interconnected systems are mainly focused on scalability as verifying safety becomes numerically expensive with the dimension of the system.

In the context of interconnected system, an interesting question is whether or how the individual sub-systems and their interactions play role in satisfying or violating a given safety constraint. Specifically in complex CPS, as the sub-systems have distinct dynamics in variant time-scale, failure or attack in one sub-system may have significantly different impact to a safety constraint than the failure or attack in another. Therefore, there is an interest to quantify or bound such impacts so that they can be utilized in safety analysis and safety-critical design. Specially, knowledge of this can help to design safety-ensuring control policies in the sub-systems that are not subjected to fault or attack by compensating the impacts from faulty or attacked sub-systems. This can also guide to decide which sub-systems are more safety-critical and require higher protections.

With the above motivation, here in this paper we study safety of an interconnected system with an aim to find some indices for the sub-systems that are vulnerable to fault or attack, which then can be leveraged to compute safety-ensuring control policies in the non-vulnerable sub-systems. We take barrier function based approach for our study. In this paper we make the following contributions:

\begin{itemize}

\item We define two types of indices for the sub-systems that are vulnerable to failure or attack. One type of indices capture the worst-case impacts on the safety constraints from the self-dynamics of each vulnerable sub-system whereas the other one captures the worst-case impact from the the coupled dynamics of the vulnerable sub-systems.

\item Utilizing the defined indices we then derive a sufficient condition for the control policies in the non-vulnerable sub-systems that compensate the impacts of fault/attack in the vulnerable sub-systems so that the given safety constraints are satisfied. 

\item We provide algorithms based on sum-of-squares optimization to compute the defined indices and the safety-ensuring control policies in the non-vulnerable sub-systems. We also discuss two special cases where more simpler and computationally efficient methods can be used to the find the indices.

\item We present a case study of temperature regulation of interconnected rooms to illustrate our results.

\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control policies. Section \ref{sec:algo} presents the algorithms for computing control polices and the indices. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> introduction_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Cyber-physical systems (CPS) are vulnerable to random failures and cyber-attacks which can potentially cause damage to the system and even endanger human lives. Therefore CPS especially critical infrastructure are required to maintain safety even under failures or attacks.
Cyber-physical Systems (CPS) \cite{ames2016control,cohen2020approximate,fan2020fast} have been shown to be vulnerable to random failures and cyber-attacks, which can cause safety violations. Safety violations of CPS can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. Therefore, safe operation of CPS under fault or attack has become a priority, especially for critical infrastructures.

To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, extending these approaches to CPS consisting of multiple sub-systems and thus of higher complexities and larger scales is non-trivial. The reason is that the interconnected sub-systems may have distinct dynamics in variant time-scales, failure or attack in one sub-system can thus have significantly different impact to a safety constraint than the failure or attack in another. Therefore, an intelligent adversary can degrade the system performance and cause safety violation by compromising only a subset of interconnected sub-systems. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems since an intelligent adversary can explore the vulnerabilities not only in each sub-system, but also in the interconnections among the sub-systems to attack the CPS. In addition, CPS with multiple interconnected sub-systems may have multiple distinct safety requirements.


Consider an interconnected CPS consisting of multiple sub-systems under a set of distinct safety constraints. When a subset of sub-systems incurs faults or is compromised by a malicious adversary, we desire a metric to quantify the impacts introduced by the interconnections among the sub-systems so as to verify if the CPS can isolate or tolerate the faulty and compromised sub-systems without weakening the safety guarantee. However, designing and computing such metric is not straightforward since the dimension of the state and action spaces increases as more sub-systems are interconnected. To the best of our knowledge, such a metric has not been proposed in the existing literature.

In this paper, we consider an interconnected CPS with multiple sub-systems with some of them being compromised by a malicious adversary. The CPS is given a set of safety constraints that needs to be satisfied by the sub-systems of the CPS. We propose a pair of indices for each sub-system that can potentially be compromised as a measure metric to capture its impact on each safety constraint. 
%The first index quantifies the impact of the sub-system when there exists no interconnection, and the second index models the impact introduced by the interconnection. 
Using our proposed indices, one can design a control law for a subset of sub-systems that are fault- and attack-free to satisfying the safety constraint while the others become compromised. The control synthesis needs to satisfy a set of constraints that is linear in the number of sub-systems. Both proposed indices are scalars, making the safety verification and design of control law more tractable than directly working in the high-dimensional state space of the CPS. In this paper we make the following contributions:



% Many of efforts for interconnected systems are mainly focused on scalability as verifying safety becomes numerically expensive with the dimension of the system.

% In the context of interconnected system, an interesting question is whether or how the individual sub-systems and their interactions play role in satisfying or violating a given safety constraint. Specifically in complex CPS, as the sub-systems have distinct dynamics in variant time-scale, failure or attack in one sub-system may have significantly different impact to a safety constraint than the failure or attack in another. Therefore, there is an interest to quantify or bound such impacts so that they can be utilized in safety analysis and safety-critical design. Specially, knowledge of this can help to design safety-ensuring control policies in the sub-systems that are not subjected to fault or attack by compensating the impacts from faulty or attacked sub-systems. This can also guide to decide which sub-systems are more safety-critical and require higher protections.

% With the above motivation, here in this paper we study safety of an interconnected system with an aim to find some indices for the sub-systems that are vulnerable to fault or attack, which then can be leveraged to compute safety-ensuring control policies in the non-vulnerable sub-systems. In this paper we make the following contributions:

\begin{itemize}

\item We define a pair of indices for the sub-systems that are vulnerable to failure or attack. The first index quantifies the impact of the sub-system when there exists no interconnection, and the second index models the impact introduced by the interconnection. 

\item Utilizing the proposed indices, we then derive a sufficient condition for the control policies in the remaining sub-systems that compensate the impacts of fault/attack in the vulnerable sub-systems so that the given safety constraints are satisfied. 

\item We propose an algorithm based on sum-of-squares optimization to compute the proposed indices and the safety-ensuring control policies. We also discuss two special cases where more computationally efficient methods can be developed to the find the indices.

\item We present a case study of temperature regulation of interconnected rooms to illustrate our results.

\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control policies. Section \ref{sec:algo} presents the algorithms for computing control polices and the indices. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> introduction_v3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Cyber-physical Systems (CPS) \cite{ames2016control,cohen2020approximate,fan2020fast} have been shown to be vulnerable to random failures and cyber attacks, which can cause safety violations. Safety violations of CPS can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. Therefore, safe operation of CPS under fault or attack has become a priority, especially for critical infrastructures.

To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, these approaches are not readily extendable to complex CPS with interconnected sub-systems. 
Addition of new sub-systems increases the dimension of the system and may introduce heterogeneity which makes approaches designed for low-dimensional and homogeneous systems intractable. Besides, complex attack scenarios are possible in interconnected sub-systems where adversaries can adopt different attack strategies on each sub-system making certain defense or resilient approaches ineffective. In addition, the interconnections of sub-systems can be unreliable which in consequence increases vulnerability to attacks. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.



%However, safety analysis and control of safety-critical CPS become challenging as the complexity and scale of CPS increase. Specifically, CPS with multiple interconnected sub-systems may have multiple distinct safety requirements. In addition, as more sub-systems are interconnected, the system dimension increases, making some existing approaches designed for low-dimensional system intractable. Furthermore, an intelligent adversary can utilize additional surfaces to attack the system as more sub-systems are interconnected. A comprehensive protection against attack over entire system may be impractical for large-scale CPS. 



%However, extending these approaches to CPS consisting of multiple sub-systems and thus of higher complexities and larger scales is non-trivial. The reason is that the interconnected sub-systems may have distinct dynamics in variant time-scales, failure or attack in one sub-system can thus have significantly different impact to a safety constraint than the failure or attack in another. Therefore, an intelligent adversary can degrade the system performance and cause safety violation by compromising only a subset of interconnected sub-systems. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems since an intelligent adversary can explore the vulnerabilities not only in each sub-system, but also in the interconnections among the sub-systems to attack the CPS. In addition, CPS with multiple interconnected sub-systems may have multiple distinct safety requirements.


%Consider an interconnected CPS consisting of multiple sub-systems under a set of distinct safety constraints. When a subset of sub-systems incurs faults or is compromised by a malicious adversary, we desire a metric to quantify the impacts introduced by the interconnections among the sub-systems so as to verify if the CPS can isolate or tolerate the faulty and compromised sub-systems without weakening the safety guarantee. However, designing and computing such metric is not straightforward since the dimension of the state and action spaces increases as more sub-systems are interconnected. To the best of our knowledge, such a metric has not been proposed in the existing literature.

%In the context of interconnected system, an interesting question is whether or how the individual sub-systems and their interactions play role in satisfying or violating a given safety constraint. Specifically in complex CPS, as the sub-systems have distinct dynamics in variant time-scale, failure or attack in one sub-system may have significantly different impact to a safety constraint than the failure or attack in another. Therefore, there is an interest to quantify or bound such impacts so that they can be utilized in safety analysis and safety-critical design. Specially, knowledge of this can help to design safety-ensuring control policies in the sub-systems that are not subjected to fault or attack by compensating the impacts from faulty or attacked sub-systems. This can also guide to decide which sub-systems are more safety-critical and require higher protections.

Considering above, it is of interest to guarantee safety of an interconnected sub-systems when some sub-systems are subject to fault and attack. However, the impact of fault or attack in each sub-system may be significantly different to a given safety constraint because the sub-systems usually have distinct dynamics in variant time-scale. Thereby it is desirable to find some indices that quantify the impacts of compromised or faulty sub-systems to a safety constraint so that these indices can be leveraged in the safety analysis and safety-critical design. Development of such indices will also guide in deciding which sub-systems are more safety-critical and require better protections. However, finding such indices is not trivial and remains an open problem.   



%In this paper, we consider an interconnected CPS with multiple sub-systems with some of them being subject to faults or malicious attacks. The CPS is given a set of safety constraints that needs to be satisfied by the sub-systems of the CPS. We propose a pair of indices for each sub-system that can potentially be compromised as a measure metric to capture its impact on each safety constraint. 
%The first index quantifies the impact of the sub-system when there exists no interconnection, and the second index models the impact introduced by the interconnection. 
%Using our proposed indices, one can design a control law for a subset of sub-systems that are fault- and attack-free to satisfying the safety constraint while the others become compromised. The control synthesis needs to satisfy a set of constraints that is linear in the number of sub-systems. Both proposed indices are scalars, making the safety verification and design of control law more tractable than directly working in the high-dimensional state space of the CPS. In this paper we make the following contributions:


In this paper, we consider an interconnected CPS with multiple sub-systems where some of them are subject to faults or malicious attacks. A set of safety constraints is given that needs to be satisfied by the CPS. We propose indices for each faulty/compromised sub-system to bound its impact on the safety constraints. Using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free so that the safety constraints are satisfied. The indices can be computed off-line and the proposed design for control laws is scalable to high-dimensional CPS. In this paper we make the following contributions:

% With the above motivation, here in this paper we study safety of an interconnected system with an aim to find some indices for the sub-systems that are vulnerable to fault or attack, which then can be leveraged to compute safety-ensuring control policies in the non-vulnerable sub-systems. In this paper we make the following contributions:

\begin{itemize}

\item We define two types of indices for the sub-systems that are vulnerable to failure or attack. The first type quantifies the impact of the sub-system when there exists no interconnection, and the second one models the impact introduced by the interconnections. 

\item Utilizing the proposed indices, we then derive a sufficient condition for the control laws in the remaining sub-systems that compensate the impacts of fault/attack in the vulnerable sub-systems so that the given safety constraints are satisfied. 

\item We propose an algorithm based on sum-of-squares optimization to compute the proposed indices and the safety-ensuring control policies. We also discuss two special cases where more computationally efficient methods can be developed to the find the indices.

\item We present a case study of temperature regulation of interconnected rooms to illustrate our results.

\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control laws. Section \ref{sec:algo} presents the algorithms for computing the indices and synthesizing the control laws. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> introduction_v4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Cyber-physical Systems (CPS) \cite{ames2016control,cohen2020approximate,fan2020fast} have been shown to be vulnerable to random failures and cyber attacks, which can cause safety violations. Safety violations of CPS can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. Therefore, safe operation of CPS under fault or attack has become a priority, especially for critical infrastructures. To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}.


Safety analysis and safety-critical control of interconnected sub-systems are challenging and require further efforts. Dimension of the system grows with the number of sub-systems which makes approaches designed for low-dimensional systems intractable for interconnected sub-systems . This motivates compositional approaches for safety verification \cite{?}. However, in interconnected sub-systems complex attack scenarios are possible where adversaries can adopt different attack strategies in different sub-systems. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, these approaches are not readily extendable to complex CPS with interconnected sub-systems. 
%Addition of new sub-systems increases the dimension of the system and may introduce heterogeneity which makes approaches designed for low-dimensional and homogeneous systems intractable. Besides, complex attack scenarios are possible in interconnected sub-systems where adversaries can adopt different attack strategies on each sub-system making certain defense or resilient approaches ineffective. In addition, the interconnections of sub-systems can be unreliable which in consequence increases vulnerability to attacks. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%Considering above, it is of interest to guarantee safety of an interconnected sub-systems when some sub-systems are subject to fault and attack. However, the impact of fault or attack in each sub-system may be significantly different to a given safety constraint because the sub-systems usually have distinct dynamics in variant time-scale. Thereby it is desirable to find some indices that quantify the impacts of compromised or faulty sub-systems to a safety constraint so that these indices can be leveraged in the safety analysis and safety-critical design. Development of such indices will also guide in deciding which sub-systems are more safety-critical and require better protections. However, finding such indices is not trivial and remains an open problem.   

Considering above, it is of interest to develop solution for safety-critical control in an interconnected sub-systems when some of the sub-systems are subject to fault and attack. One way to develop such solution is to simplify the design utilizing some indices that bounds the impacts of compromised or faulty sub-systems on given safety constraints. This design approach based on safety indices will not only provide better scalability but also allow higher flexibility to each fault- or attack-free sub-system in its design of own control laws. However, finding such indices is not trivial and remains an open problem in the context of safety of interconnected systems . 

%In this paper, we consider an interconnected CPS with multiple sub-systems where some of them are subject to faults or malicious attacks. A set of safety constraints is given that needs to be satisfied by the CPS. We propose indices for each faulty/compromised sub-system to bound its impact on the safety constraints. Using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free so that the safety constraints are satisfied. The indices can be computed off-line and the proposed design for control laws is scalable to high-dimensional CPS. In this paper we make the following contributions:

Motivated by above, in this paper we aim to develop safety-critical control laws by finding some indices for safety in an interconnected sub-systems where some of sub-systems are faulty or compromised. We propose indices that bounds impact of each faulty/compromised and allows us to form compositional control barrier functions. Using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free so that given safety constraints are satisfied. The indices can be computed off-line and the proposed design for control laws is scalable to high-dimensional CPS. In this paper we make the following contributions:


\begin{itemize}

\item We define two types of indices for the sub-systems that are vulnerable to failure or attack. The first type quantifies the worst-case impact of the sub-system on safety constraints when there exists no interconnection, and the second one models the worst-case impact introduced by the interconnections. 

\item Utilizing the proposed indices, we then derive a sufficient condition for the control laws in the remaining sub-systems that compensate the impacts of fault/attack in the vulnerable sub-systems so that the given safety constraints are satisfied. 

\item We propose an algorithm based on sum-of-squares optimization to compute the proposed indices and the safety-ensuring control policies. We also discuss two special cases where more computationally efficient methods can be developed to the find the indices.

\item We present a case study of temperature regulation of interconnected rooms to illustrate our results.

\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control laws. Section \ref{sec:algo} presents the algorithms for computing the indices and synthesizing the control laws. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> introduction_v5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Cyber-physical Systems (CPS) \cite{ames2016control,cohen2020approximate,fan2020fast} have been shown to be vulnerable to random failures and cyber attacks, which can cause safety violations. Safety violations of CPS can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. Therefore, safe operation of CPS under fault or attack has become a priority, especially for critical infrastructures. To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}.


Resilient and safety-critical control is especially challenging for CPS that are formed by the interconnection of subsystems. In such CPS, safety constraints can be imposed on the overall system and/or individual sub-systems. Due to the interconnections among the sub-systems, faults and attacks in one sub-system may lead to safety violation in others and the overall CPS \cite{yang2020exponential,yang2015fault}. Thus, an intelligent adversary can employ different attack strategies in different sub-systems to compromise the controllers to cause safety violations and maximize the damage. In addition, the dimension of interconnected CPS grows with the number of sub-systems, which poses a scalability challenge. 
% As a consequence, safety verification and comprehensive protection over the entire CPS become less practical.


% Dimension of the system grows with the number of sub-systems which makes approaches designed for low-dimensional systems intractable for interconnected sub-systems. This motivates compositional approaches for safety verification \cite{?}. However, in interconnected sub-systems complex attack scenarios are possible where adversaries can adopt different attack strategies in different sub-systems. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, these approaches are not readily extendable to complex CPS with interconnected sub-systems. 
%Addition of new sub-systems increases the dimension of the system and may introduce heterogeneity which makes approaches designed for low-dimensional and homogeneous systems intractable. Besides, complex attack scenarios are possible in interconnected sub-systems where adversaries can adopt different attack strategies on each sub-system making certain defense or resilient approaches ineffective. In addition, the interconnections of sub-systems can be unreliable which in consequence increases vulnerability to attacks. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%Considering above, it is of interest to guarantee safety of an interconnected sub-systems when some sub-systems are subject to fault and attack. However, the impact of fault or attack in each sub-system may be significantly different to a given safety constraint because the sub-systems usually have distinct dynamics in variant time-scale. Thereby it is desirable to find some indices that quantify the impacts of compromised or faulty sub-systems to a safety constraint so that these indices can be leveraged in the safety analysis and safety-critical design. Development of such indices will also guide in deciding which sub-systems are more safety-critical and require better protections. However, finding such indices is not trivial and remains an open problem.   

% To address these challenges, it is of interest to develop scalable solutions for safety-critical control in interconnected systems when some of the sub-systems are possibly subject to fault and attack. Recently compositional approaches have been proposed for interconnected systems \cite{}

To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity}. These approaches do not consider the presence of fault or attack. A compositional fault-tolerant scheme was recently proposed in \cite{yang2020exponential}. However, compositional fault- and intrusion-tolerant safety-critical for interconnected CPS has been less studied. Indices that bound the impacts of compromised/faulty sub-systems on the given safety constraints can significantly simplify the solution. Moreover, such safety indices will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that are not trivial and remains an open problem in the context of safety of interconnected systems. 


% To alleviate the scalability challenge, compositional approaches have been proposed that decompose the safety constraint over the sub-systems in the absence of fault or attack. \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity}. It is also of interest to develop compositional solution for safety-critical control when some of the sub-systems are subject to fault and attack. Indices that bound the impacts of compromised/faulty sub-systems on the given safety constraints can significantly simplify the solution. Moreover, such safety indices will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that are not trivial and remains an open problem in the context of safety of interconnected systems. 


% To address the challenges above, it is of interest to develop solution for safety-critical control in an interconnected systems when some of the sub-systems are subject to fault and attack. One way to develop such solution is to simplify the design utilizing some indices that bounds the impacts of compromised or faulty sub-systems on given safety constraints. This design approach based on safety indices will not only provide better scalability but also allow higher flexibility when designing and replacing some sub-systems. However, finding such indices is not trivial and remains an open problem in the context of safety of interconnected systems. 

%In this paper, we consider an interconnected CPS with multiple sub-systems where some of them are subject to faults or malicious attacks. A set of safety constraints is given that needs to be satisfied by the CPS. We propose indices for each faulty/compromised sub-system to bound its impact on the safety constraints. Using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free so that the safety constraints are satisfied. The indices can be computed off-line and the proposed design for control laws is scalable to high-dimensional CPS. In this paper we make the following contributions:

In this paper, we aim to develop safety critical control laws for interconnected systems in which some of the subsystems are faulty or compromised. Our proposed approach is based on constructing/formulating indices that describe the impact of each subsystem on the overall safety. We propose indices to bound the impact of each faulty/compromised sub-system  on the safety constraints. Using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free so that given safety constraints are satisfied. The conditions are derived by formulating a control barrier function based constraint for each sub-system. The indices can be computed off-line and the proposed design for control laws is scalable to high-dimensional CPS. In this paper we make the following contributions:


\begin{itemize}

\item We define two types of indices for the sub-systems that are vulnerable to failure or attack. The first type quantifies the worst-case impact of the sub-system on safety constraints when there exists no interconnection, and the second one models the worst-case impact introduced by the interconnections. 

\item Utilizing the proposed indices, we then derive a sufficient condition for the control laws in the remaining sub-systems to compensate for the impacts of fault/attack in the vulnerable sub-systems so that the given safety constraints are satisfied. 

\item We propose an algorithm based on sum-of-squares optimization to compute the proposed indices and the safety-ensuring control policies. We also discuss two special cases where more computationally efficient methods can be developed to the find the indices.

\item We present a case study of temperature regulation of interconnected rooms to illustrate our results in two scenarios where safety is defined on the overall system or each individual room. We demonstrate that our proposed approach guarantees safety in both scenarios.

\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control laws. Section \ref{sec:algo} presents the algorithms for computing the indices and synthesizing the control laws. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> introduction_v6.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Safety is an important property of cyber-physical systems (CPS) in multiple domains including power systems and transportation \cite{ames2016control,cohen2020approximate,fan2020fast}. Safety violations can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. To this end, safety verification and safety-critical control for CPS have been extensively studied \cite{ames2016control,cohen2020approximate,xu2018constrained,prajna2007framework}.

CPS have been shown to be vulnerable to random failures and cyber attacks, which can cause safety violations \cite{sullivan2017cyber,Jeep}. To mitigate the impacts of faults and cyber attacks, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. Resilient and safety-critical control can be even more challenging for the class of CPS that are formed by the interconnection of sub-systems \cite{rinaldi2001identifying,zhang2019robustness}. 
% In such CPS, safety constraints can be imposed on the overall system and/or individual sub-systems. 
Due to the interdependencies among the sub-systems, faults and attacks in one sub-system may lead to safety violation in others and the overall CPS. For instance, a local and small disturbance was escalated by the interconnection of the power system, causing the blackout in India in 2012 \cite{india}. Thus, an intelligent adversary can utilize such cascading effects underlying the interactions among the sub-systems to compromise the controllers and cause maximum-impact safety violations. In addition, the dimension of interconnected CPS grows with the number of sub-systems, which poses a scalability challenge in safety verification and safety-critical control design. 
% As a consequence, safety verification and comprehensive protection over the entire CPS become less practical.


% Dimension of the system grows with the number of sub-systems which makes approaches designed for low-dimensional systems intractable for interconnected sub-systems. This motivates compositional approaches for safety verification \cite{?}. However, in interconnected sub-systems complex attack scenarios are possible where adversaries can adopt different attack strategies in different sub-systems. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, these approaches are not readily extendable to complex CPS with interconnected sub-systems. 
%Addition of new sub-systems increases the dimension of the system and may introduce heterogeneity which makes approaches designed for low-dimensional and homogeneous systems intractable. Besides, complex attack scenarios are possible in interconnected sub-systems where adversaries can adopt different attack strategies on each sub-system making certain defense or resilient approaches ineffective. In addition, the interconnections of sub-systems can be unreliable which in consequence increases vulnerability to attacks. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%Considering above, it is of interest to guarantee safety of an interconnected sub-systems when some sub-systems are subject to fault and attack. However, the impact of fault or attack in each sub-system may be significantly different to a given safety constraint because the sub-systems usually have distinct dynamics in variant time-scale. Thereby it is desirable to find some indices that quantify the impacts of compromised or faulty sub-systems to a safety constraint so that these indices can be leveraged in the safety analysis and safety-critical design. Development of such indices will also guide in deciding which sub-systems are more safety-critical and require better protections. However, finding such indices is not trivial and remains an open problem.   

% To address these challenges, it is of interest to develop scalable solutions for safety-critical control in interconnected systems when some of the sub-systems are possibly subject to fault and attack. Recently compositional approaches have been proposed for interconnected systems \cite{}

%To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity,yang2015fault,yang2020exponential}. These approaches do not consider the presence of attack. To the best of our knowledge, compositional fault- and intrusion-tolerant safety-critical control for interconnected CPS has been less studied. To develop such compositional fault- and intrusion-tolerant approach, one needs to identify some measure indices to model how faults and attacks propagate in CPS via interactions to yield safety violations. By using the indices, it will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that remain an open problem in the context of safety of interconnected systems. 


%To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity,yang2015fault,yang2020exponential}. These approaches do not consider the presence of attack. To the best of our knowledge, compositional fault- and intrusion-tolerant safety-critical control for interconnected CPS has been less studied. To develop such compositional fault- and intrusion-tolerant approach, one needs to identify some measure indices to model how faults and attacks propagate in CPS via interactions to yield safety violations. By using the indices, it will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that remain an open problem in the context of safety of interconnected systems.

To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity,yang2015fault,yang2020exponential}. These approaches do not consider the presence of attack. Specifically, compositional approach to fault- and intrusion-tolerant safety-critical control for interconnected CPS has received limited research attention. Development of such approach for safety-critical control necessitates to identify some measure indices to model how faults and attacks propagate in CPS via interactions to yield safety violations. Usage of such indices will also allow higher flexibility in designing safety-ensuring control in each sub-system. However, finding such indices and designing control based upon that remain an open problem in the context of safety of interconnected systems.

% To alleviate the scalability challenge, compositional approaches have been proposed that decompose the safety constraint over the sub-systems in the absence of fault or attack. \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity}. It is also of interest to develop compositional solution for safety-critical control when some of the sub-systems are subject to fault and attack. Indices that bound the impacts of compromised/faulty sub-systems on the given safety constraints can significantly simplify the solution. Moreover, such safety indices will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that are not trivial and remains an open problem in the context of safety of interconnected systems. 


% To address the challenges above, it is of interest to develop solution for safety-critical control in an interconnected systems when some of the sub-systems are subject to fault and attack. One way to develop such solution is to simplify the design utilizing some indices that bounds the impacts of compromised or faulty sub-systems on given safety constraints. This design approach based on safety indices will not only provide better scalability but also allow higher flexibility when designing and replacing some sub-systems. However, finding such indices is not trivial and remains an open problem in the context of safety of interconnected systems. 

%In this paper, we consider an interconnected CPS with multiple sub-systems where some of them are subject to faults or malicious attacks. A set of safety constraints is given that needs to be satisfied by the CPS. We propose indices for each faulty/compromised sub-system to bound its impact on the safety constraints. Using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free so that the safety constraints are satisfied. The indices can be computed off-line and the proposed design for control laws is scalable to high-dimensional CPS. In this paper we make the following contributions:

%In this paper, we aim to develop safety-critical control laws for interconnected systems in which some of the sub-systems are faulty or compromised. Our proposed approach is based on constructing indices that bound the impact of each subsystem on the overall safety. By using our proposed indices, we give conditions to design control laws for the remaining sub-systems that are fault- and attack-free by constructing a control barrier function based constraint. In this paper we make the following contributions:

In this paper, we aim to develop safety-critical control laws for interconnected systems in which some of the sub-systems are faulty or compromised. We consider a class of interconnected systems  where the dynamics of each sub-system are coupled to others. Our proposed approach is based on constructing indices that bound the impacts of each subsystem on the specified safety constraints. Using the proposed indices as well as control barrier functions,  we provide conditions and algorithm to design control laws for the remaining sub-systems that are fault- and attack-free. We make the following contributions:


\begin{itemize}

\item We define two types of indices for the sub-systems that are vulnerable to failure or attack. The first type quantifies the worst-case impact of the sub-system on safety constraints when there exists no coupling, and the second one models the worst-case impact introduced by the couplings. 

\item Utilizing the proposed indices, we then derive a sufficient condition for the safety-ensuring control policies in the fault- and attack-free sub-systems that compensate the impacts of faults and attacks in the vulnerable sub-systems.

%\item We propose an algorithm based on sum-of-squares optimization that compute the proposed indices and the safety-ensuring control policies. We prove that the synthesized control policies guarantees system safety. We discuss two special cases on linear systems and monotone systems, where less computationally expensive methods can be used to the find the indices.

\item We propose an algorithm based on sum-of-squares optimization that computes the proposed indices and the safety-ensuring control policy in each fault- and attack-free sub-system independently. We discuss two special cases on linear systems and monotone systems, where computationally efficient methods can be used to find the indices.

%\item We present a case study of temperature regulation of interconnected rooms to illustrate our results in two scenarios where safety is defined on the overall system or each individual room. We demonstrate that our proposed approach guarantees safety in both scenarios.

\item We present a case study of temperature regulation of interconnected rooms to illustrate our approach. We demonstrate that the control policy obtained using our algorithm maintains the specified safety constraints. 
\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control policies. Section \ref{sec:algo} presents the algorithms for computing the indices and synthesizing the control policies. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> introduction_v7.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Safety is an important property of cyber-physical systems (CPS) in multiple domains including power systems and transportation \cite{ames2016control,cohen2020approximate,fan2020fast}. Safety violations can potentially cause damage to the system and even endanger human lives \cite{sullivan2017cyber,Jeep}. To this end, safety verification and safety-critical control for CPS have been extensively studied \cite{ames2016control,cohen2020approximate,xu2018constrained,prajna2007framework}.

CPS have been shown to be vulnerable to random failures and cyber attacks, which can cause safety violations \cite{sullivan2017cyber,Jeep}. To mitigate the impacts of faults and cyber attacks, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. Resilient and safety-critical control can be even more challenging for the class of CPS that are formed by the interconnection of sub-systems \cite{rinaldi2001identifying,zhang2019robustness}. 
% In such CPS, safety constraints can be imposed on the overall system and/or individual sub-systems. 
Due to the interdependencies among the sub-systems, faults and attacks in one sub-system may lead to safety violation in others and the overall CPS. For instance, a local and small disturbance was escalated by the interconnection of the power system, causing the blackout in India in 2012 \cite{india}. Thus, an intelligent adversary can utilize such cascading effects underlying the interactions among the sub-systems to compromise the controllers and cause maximum-impact safety violations. In addition, the dimension of interconnected CPS grows with the number of sub-systems, posing a scalability challenge in safety verification and safety-critical control design. 
% As a consequence, safety verification and comprehensive protection over the entire CPS become less practical.


% Dimension of the system grows with the number of sub-systems which makes approaches designed for low-dimensional systems intractable for interconnected sub-systems. This motivates compositional approaches for safety verification \cite{?}. However, in interconnected sub-systems complex attack scenarios are possible where adversaries can adopt different attack strategies in different sub-systems. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%To this end, defense against attacks, fault-tolerant designs, and resilient control for CPS have garnered significant research attention \cite{bjorck2015cyber,zhu2015game,ivanov2016attack,fawzi2014secure}. However, these approaches are not readily extendable to complex CPS with interconnected sub-systems. 
%Addition of new sub-systems increases the dimension of the system and may introduce heterogeneity which makes approaches designed for low-dimensional and homogeneous systems intractable. Besides, complex attack scenarios are possible in interconnected sub-systems where adversaries can adopt different attack strategies on each sub-system making certain defense or resilient approaches ineffective. In addition, the interconnections of sub-systems can be unreliable which in consequence increases vulnerability to attacks. Although a comprehensive protection against attacks over the entire CPS may prevent sub-systems from being compromised, this approach is in general impractical for large-scale systems.


%Considering above, it is of interest to guarantee safety of an interconnected sub-systems when some sub-systems are subject to fault and attack. However, the impact of fault or attack in each sub-system may be significantly different to a given safety constraint because the sub-systems usually have distinct dynamics in variant time-scale. Thereby it is desirable to find some indices that quantify the impacts of compromised or faulty sub-systems to a safety constraint so that these indices can be leveraged in the safety analysis and safety-critical design. Development of such indices will also guide in deciding which sub-systems are more safety-critical and require better protections. However, finding such indices is not trivial and remains an open problem.   

% To address these challenges, it is of interest to develop scalable solutions for safety-critical control in interconnected systems when some of the sub-systems are possibly subject to fault and attack. Recently compositional approaches have been proposed for interconnected systems \cite{}

%To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity,yang2015fault,yang2020exponential}. These approaches do not consider the presence of attack. To the best of our knowledge, compositional fault- and intrusion-tolerant safety-critical control for interconnected CPS has been less studied. To develop such compositional fault- and intrusion-tolerant approach, one needs to identify some measure indices to model how faults and attacks propagate in CPS via interactions to yield safety violations. By using the indices, it will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that remain an open problem in the context of safety of interconnected systems. 


%To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity,yang2015fault,yang2020exponential}. These approaches do not consider the presence of attack. To the best of our knowledge, compositional fault- and intrusion-tolerant safety-critical control for interconnected CPS has been less studied. To develop such compositional fault- and intrusion-tolerant approach, one needs to identify some measure indices to model how faults and attacks propagate in CPS via interactions to yield safety violations. By using the indices, it will also allow higher flexibility when designing control. However, finding such indices and designing control based upon that remain an open problem in the context of safety of interconnected systems.

To alleviate the scalability challenge, compositional approaches which decompose the safety constraint over the sub-systems have been proposed \cite{nejati2020compositional,sloth2012compositional,lyu2022small,coogan2014dissipativity,yang2015fault,yang2020exponential}. These approaches do not consider the presence of attack. Specifically, compositional approach to fault- and intrusion-tolerant safety-critical control for interconnected CPS has received limited research attention. 


%Finding scalable solution that allows flexible design for safety-ensuring control policies is still an open problem. The present paper aims to fill this gap.

% Development of such approach for safety-critical control necessitates to identify some measure indices to model how faults and attacks propagate in CPS via interactions to yield safety violations. Usage of such indices will also allow higher flexibility in designing safety-ensuring control in each sub-system. However, finding such indices and designing control based upon that remain an open problem in the context of safety of interconnected systems.


In this paper, we aim to develop a compositional approach to safety-critical control for interconnected systems in which some of the sub-systems are faulty or compromised. We consider a class of interconnected systems where the dynamics of each sub-system are coupled to others. We propose an {\it intrinsic resilient-safety index} and a {\it coupled resilient-safety index} using the self- and coupled-dynamics of each sub-system, respectively. Using the proposed indices as well as control barrier functions, we provide conditions and algorithm to design control laws for the remaining sub-systems that are fault- and attack-free. We make the following contributions:


%In this paper, we aim to develop a compositional approach to safety-critical control for interconnected systems in which some of the sub-systems are faulty or compromised. We consider a class of interconnected systems where the dynamics of each sub-system are coupled to others. Our proposed approach is based on constructing indices that bound the impacts of each subsystem on the specified safety constraints. Using the proposed indices as well as control barrier functions, we provide conditions and algorithm to design control laws for the remaining sub-systems that are fault- and attack-free. We make the following contributions:


\begin{itemize}

\item We define intrinsic resilient-safety and coupled resilient-safety indices for the sub-systems that are vulnerable to failure or attack. The intrinsic resilient-safety index bounds the worst-case impact of the sub-system on safety constraint due to intrinsic/self-dynamics, whereas the coupled resilient-safety, bounds the worst-case impact introduced by the couplings. 

\item Utilizing the proposed indices, we derive a sufficient condition for the safety-ensuring control policies in the fault- and attack-free sub-systems that compensate the impacts of faults and attacks in the vulnerable sub-systems.

\item We propose an algorithm based on sum-of-squares optimization that computes the proposed indices and the safety-ensuring control policy in each fault- and attack-free sub-system independently. We discuss two special cases on linear systems and monotone systems, where computationally efficient methods can be used to find the indices.
\item We present a case study of temperature regulation of interconnected rooms to illustrate our approach. We demonstrate that the control policy obtained using our algorithm maintains the specified safety constraints. 
\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:related} presents the related works. Section \ref{sec:formulation} presents the system model and formulates the problem. Section \ref{sec:Res} introduces the indices and presents the condition for safety-ensuring control policies. Section \ref{sec:algo} presents the algorithms for computing the indices and synthesizing the control policies. Section \ref{sec:simulation} contains a case study. Section \ref{sec:conclusion} concludes the paper.





==> result.tex <==
\section{Main Result}\label{sec:Res}

In this section we present our main results. First we present our solution approach for finding the control policies that guarantee safety. Then we present algorithms for computing the control policies and the associated parameters.

\subsection{Solution Approach}

In this section we develop a solution for Problem \ref{prob1}. In our solution approach, we first derive some indices which relate to the worst-case impacts on the safety constraints caused by the individual self-dynamics and the coupled-dynamics of the vulnerable subsystems. Based on these indices we then obtain the sufficient conditions for control policy in the protected subsystems so that safety constraints are guaranteed irrespective of the condition (i.e. whether faulty/compromised or not) of any of the vulnerable subsystems.

\begin{definition}[]\label{def:monotone}
Consider index  $\hat{\gamma}_i^k\in\mathbb{R}$ for each $i \in \mathcal{N}_2$ and $k=1,\ldots,K$ such that 
\begin{equation}\label{eq:gamma1}
\hat{\gamma}_i^k = \inf_{x\in\mathcal{C}, u_i\in\mathcal{U}_i} \left\{\frac{\partial h^k}{\partial x_i}(f_{i,self}(x_i)+g_{i,self}(x_i)u_i)\right\} 
\end{equation}
\end{definition}
The parameter $\hat{\gamma}_i^k$ bounds the worst-case impact from the self-dynamics of sub-system $\mathcal{S}_i$ on the safety constraint $h^k(x) \geq 0$. For instance, $\hat{\gamma}_i^k\geq 0$ indicates that self-dynamics of sub-system $\mathcal{S}_i$ does not contribute to the safety violation of constraint $h^k(x) \geq 0$ for any $u_i\in\mathcal{U}_i$. However, when $\hat{\gamma}_i^k$ is not available or not easy to compute, we instead $\gamma_i^k\in\mathbb{R}$ such that
\begin{equation}\label{eq:gamma}
    \frac{\partial h^k}{\partial x_i}(f_{i,self}(x_i)+g_{i,self}(x_i)u_i) \geq \gamma_i^k
\end{equation}
From definition, it is clear that from definition that for any $\gamma_i^k$ satisfying \eqref{eq:gamma}, $\hat{\gamma}_i^k \geq \gamma_i^k$. Thus  $\hat{\gamma}_i^k$ renders the inequality \eqref{eq:gamma} to be the tightest.

We further define $\beta^k \in \mathbb{R}$ for $k=1,\ldots,K$ such that following holds for all $x\in\mathcal{C}$ and $u_i\in\mathcal{U}_i$.
\begin{equation}\label{eq:beta}
\sum_{i=m+1}^N\frac{\partial h^k}{\partial x_i}(f_{i,coupled}(x_i,x_{-i}) +g_{i,coupled}(x_i,x_{-i})u_i) \geq \beta^k
\end{equation}
Similar to $\gamma_i^k$, the parameter $\beta^k$ bounds the worst-case impact from vulnerable subsystems $\mathcal{N}_2$ towards violating the safety constraint of $h^k(x) \geq 0$ for their coupled-dynamics. Here one can also choose $\beta^k$ to be the infimum of the left hand side expressions of \eqref{eq:beta} i.e. $\beta^k=\hat{\beta}^k$ where $\hat{\beta}^k=\inf \Big\{\sum_{i=m+1}^N\frac{\partial h}{\partial x_i}(f_{i,coupled}(x_i,x_{-i})$ $+g_{i,coupled}(x_i,x_{-i})u_i)\Big\}$ with $x\in\mathcal{C}$ and $u_i\in \mathcal{U}_i$ for each $i \in \mathcal{N}_2$. This choice renders \eqref{eq:beta} to be the tightest. When $\beta^k\geq 0$, it indicates the coupled dynamics of vulnerable subsystems does not lead to the safety violation of constraint $h^k(x) \geq 0$.

%\begin{multline}\label{eq:beta}
%    \beta^k=\inf_{x\in\mathcal{C},\prod_{i=m+1}^Nu_i\in\prod_{i=m+1}^N\mathcal{U}_i}\%Big\{\sum_{i=m+1}^N\frac{\partial h}{\partial x_i}(f_{i,coupled}(x_i,x_{-i})\\
%    +g_{i,coupled}(x_i,x_{-i})u_i)\Big\}
%\end{multline}

Now we present our main result based on the defined parameters. This result gives a sufficient condition on control input in the protected sub-systems such that the system maintains all the safety constraints. The result is formalized below. 

\begin{theorem} \label{Th1}
Consider Problem \ref{prob1}. Suppose there exist positive constants $\alpha_i^k$ and the control input $u_i$ such that the following holds for $i \in \mathcal{N}_1$ and $k=1, \ldots, K$:
\begin{align}
     & \frac{\partial h^k}{\partial x_i}F_{i}(x_i,x_{-i},u_i)
       \geq \alpha_i^k\left(-\eta_i^k(h^k(x))-\beta^k-\sum_{j=m+1}^N\gamma_j^k\right)  \label{eq:MR}
\end{align}
where $\gamma_j^k$, $\beta^k$ are the parameters as defined before, $\eta_i^k$ is an extended class $\mathcal{K}$ function and $\sum_{i=1}^m \alpha_i^k=1$. Then the system $\mathcal{S}$ is safe with respect to $\mathcal{C}$ for all $t \geq 0$ by taking control policy $u_i$ at each $i \in \mathcal{N}_1$ given that $x(0) \in \mathcal{C}$.
\end{theorem}
\begin{proof}
$F(x,u)$ is the dynamics of system $\mathcal{S}$ and we compute $\frac{\partial h^k}{\partial x}F(x,u)$ for each $k=1,\ldots,K$ as
\begin{align}
    &\frac{\partial h^k}{\partial x}F(x,u) = \sum_{i=1}^N\frac{\partial h^k}{\partial x_i}F_i(x_i,x_{-i},u_i) \nonumber\\
    =&\sum_{i=1}^m\frac{\partial h_k}{\partial x_i}F_i(x_i,x_{-i},u_i)+\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}F_i(x_i,x_{-i},u_i)\nonumber\\
    \geq &\sum_{i=1}^m\alpha_i^k[ -\eta_i^k(h^k(x))-\beta^k-\sum_{j=m+1}^N\gamma_j^k]\nonumber\\
    &\quad+\sum_{i=m+1}^N\frac{\partial h^k}{\partial x_i}[f_{i,self}(x_i)+g_{i,self}(x_i)u_i\nonumber\\
    &\quad\quad\quad\quad\quad+f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i]\nonumber\\
    =& -\sum_{i=1}^m\alpha_i^k \eta_i^k(h^k(x)) +\sum_{i=m+1}^N\Big(\frac{\partial h^k}{\partial x_i}[f_{i,self}(x_i) \nonumber\\
    & +g_{i,self}(x_i)u_i - \gamma_i^k\Big) +\Big(\sum_{i=m+1}^N \frac{\partial h^k}{\partial x_i}[f_{i,coupled}(x_i,x_{-i}) \nonumber\\
    &\quad\quad\quad\quad\quad+g_{i,coupled}(x_i,x_{-i})u_i] - \beta^k\Big)\nonumber\\
    \geq &-\sum_{i=1}^m\alpha_i \eta_i(h^k(x)) \nonumber
\end{align}
where the last inequality holds by the definitions of $\gamma_i^k$ and $\beta^k$. Since that $\eta_i$ is an extended class $\mathcal{K}$ function and $\alpha_i\in[0,1]$, we have that $\sum_{i}\alpha_i\eta_i$ is also an extended class $K$ function. Thus $\frac{\partial h^k}{\partial x}F(x,u)\geq -\eta(h^k(x))$. Using the property of control barrier function \cite{ames2016control} and the assumption that $x(0) \in \mathcal{C}$, we have that the system remain in $\mathcal{C}^k$ for all $k=1, \dots, K$. Therefore we conclude that system $\mathcal{S}$ is safe with respect to $\mathcal{C}$.
\end{proof}

In the above theorem, the constant $\alpha_i^k$ specifies the weight on sub-system $\mathcal{S}_i$ to satisfy the safety constraint  $h^k(x) \geq 0$. As example, $\alpha_i^k=1$ means that in our approach the sub-system $\mathcal{S}_i$ is solely responsible for maintaining safety constraint $h^k(x) \geq 0$ among all the protected subsystems. $\alpha_i^k$ for $i=1, \ldots, m$ and $k=1, \ldots, K$ are chosen in a way so that the condition \eqref{eq:MR} is satisfied. One can possibly choose $\alpha_i^k$ based on the supremum of $\frac{\partial h^k}{\partial x_i}[f_{i,self}(x_i)+g_{i,self}(x_i)u_i + f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i]$.

Theorem 1 implies that if the parameters $\gamma_i^k$ and $\beta^k$ for vulnerable subsystems are known, then the control inputs in the protected subsystems to guarantee system safety can be obtained without knowing the exact models of the vulnerable sub-systems. This is useful since the control input $u_i$ employed by an adversary in a compromised sub-system is usually unknown. In this setting the above result gives a way to construct control policy in the protected sub-systems so that safety can be ensured. However, from Theorem 1 it is clear that one should use maximum possible values for $\gamma_i^k$ and $\beta^k$ (ideally $\hat{\gamma}_i^k$ and $\hat{\beta}^k$) so that the condition  \eqref{eq:MR} remains feasible. Parameters $\hat{\gamma}_i^k$ and $\hat{\beta}^k$ can be computed either numerically or analytically. Below we present a simple example for which we find the closed-form expressions for $\gamma_i^k$ and $\beta^k$ that allows us some characterization of these parameters. 

\noindent \textbf{Example:} Consider a system $\mathcal{S}:\dot{x} = Ax+Bu$ where 
\begin{equation*}
    A=\begin{bmatrix}
    a_{11}&\ldots&a_{1N}\\
    \vdots&\ddots&\vdots\\
    a_{N1}&\ldots&a_{NN}
    \end{bmatrix},\quad B=\begin{bmatrix}
    b_{11}&\ldots&0\\
    \vdots&\ddots&\vdots\\
    0&\ldots&b_{NN}
    \end{bmatrix}
\end{equation*}
Here $A \in \mathbb{R}^{n \times n}$, $B \in \mathbb{R}^{n \times n}$, $x=[x_1 \hdots x_N]^T$ and $u=[u_1 \hdots u_N]^T$. Matrix $A$ represents the system matrix for a synchronization dynamics with $a_{ii} = -\sum_{j=1, j \neq i}^N a_{ij}<0$. We consider that the system is given one ellipsoid safety constraint: $h(x)= 1- \sum_{i=1}^N c_i x_i^2$ where $c_i \geq 0$. Let the constraints on input be $|u_i| \leq 1$. Then it can be shown that $\gamma_i=-\frac{b_{ii}^2c_i}{2|a_{ii}|}$ and $\beta=- \frac{c_{max}}{c_{min}} \sum_{i=m+1}^N|a_{ii}|$ satisfy the conditions \eqref{eq:gamma} and \eqref{eq:beta} respectively, where $c_{max}$ and $c_{min}$ are the maximum and minimum values in $\{c_{m+1}. \ldots c_N\}$ respectively. The expression of $\gamma_i$ implies that $\gamma_i$ is inversely related to the magnitude of the eigenvalue of the self-dynamics of that sub-system (i.e. the higher the magnitude of eigenvalue or faster the dynamics, the lower the $\gamma_i$). The expression of $\beta$ implies that the higher the coupling (i.e. $|a_{ii}| = |\sum_{j=1, j \neq i}^N a_{ij}|$ for $i \in \mathcal{N}_2$), the higher the magnitude of $\beta$ becomes.

\subsection{Algorithmic Computation of Control Inputs}

In this section we present algorithms to compute the control policies and associated parameters $\gamma_i^k$ and $\beta_k$. Our proposed algorithms are based on the sum-of-squares optimization. Later, we present two special classes of systems for which control policies and the parameters can be computed more efficiently. 

In order to use sum-of-squares optimization, we make the following assumption on the dynamics of system and the given safety constraints.

\begin{assumption}\label{assump:semi-algebraic}
We assume that $F(x,u)$ is polynomial in $x$ and $u$, and $h^k(x)$ is polynomial in $x$ for $k=1,\ldots,K$ respectively. We further assume that $\mathcal{U}_i=\{u_i:v_i(u_i)\geq 0\}$ where $v_i$ is polynomial in $u_i$ for all $i\in\{m+1,\ldots,N\}$.
\end{assumption}

Based on the above assumption, we now present our method to compute $\hat{\gamma}_i^k$ and $\hat{\beta}^k$ using SOS optimization. For that we first show how to translate conditions \eqref{eq:gamma} and \eqref{eq:beta} into SOS constraints. We use the following result to compute $\hat{\gamma}_i^k$ for each $i\in \mathcal{N}_2$ and $k \in \{1,\ldots, K\}$.

\begin{lemma} \label{lemma:1}
Suppose Assumption \ref{assump:semi-algebraic} holds. For a sub-system  $i\in \mathcal{N}_2$ and $k \in \{1,\ldots,K\}$, if there exist sum-of-squares polynomials $p(x)$ and $q(x,u_i)$ such that $\gamma_i^k$ is the solution to the following sum-of-squares program:
\begin{subequations}\label{eq:gamma SOS}
\begin{align}
    \min_{\gamma_i^k}~ &-\gamma_i^k\\
    \st ~&\frac{\partial h^k}{\partial x_i}(f_{i,self}(x_i)+g_{i,self}(x_i)u_i)\nonumber\\
    &\quad\quad\quad-\gamma_i-p(x)h^k(x)-q(x,u_i)v_i(u_i)\geq 0\label{eq:gamma SOS 1}
\end{align}
\end{subequations}
then $\gamma_i^k$ satisfies Eqn. \eqref{eq:gamma}. Furthermore the obtained $\gamma_i^k=\hat{\gamma}_i^k$.
\end{lemma}
\begin{proof}
Let $\gamma_i^k$ be the solution to SOS program \eqref{eq:gamma SOS}. Since $p(x)$ and $q(x,u_i)$ are SOS polynomials, we have that $p(x)h^k(x)\geq 0$ for all $x\in\mathcal{C}_k$ and $q(x,u_i)v(u_i)\geq 0$ for all $u_i\in\mathcal{U}_i$. Thus $\gamma_i^k$ satisfies that
\begin{equation*}
    \gamma_i^k\leq \frac{\partial h^k}{\partial x_i}(f_{i,self}(x_i)+g_{i,self}(x_i)u_i),~\forall x\in\mathcal{C}_k,u_i\in\mathcal{U}_i
\end{equation*}
Assume that $\gamma_i^k \neq \hat{\gamma}_i^k$. Then $\hat{\gamma}_i^k>\gamma_i^k$ by the definition of $\hat{\gamma}_i^k$. Now $\hat{\gamma}_i^k$ is also feasible to constraint \eqref{eq:gamma SOS 1}. However, this contradicts the optimality of $\gamma_i$ to SOS program \eqref{eq:gamma SOS}. Hence $\gamma_i^k = \hat{\gamma}_i^k$.
\end{proof}

Similarly we use the following result to compute $\hat{\beta}^k$ for each $k\in\{1,\ldots,K\}$.
\begin{lemma}
Suppose Assumption \ref{assump:semi-algebraic} holds. If there exist sum-of-squares polynomials $p(x)$ and $q_i(x,u_i)$ such that $\beta^k$ is the solution to the following sum-of-squares program:
\begin{subequations}\label{eq:beta SOS}
\begin{align}
    \min_{\beta^k}~ &-\beta^k\\
    \st ~&\sum_{i=m+1}^N\frac{\partial h^k}{\partial x_i}(f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i)\nonumber\\
    &\quad-\beta-p(x)h^k(x)-\sum_{i=m+1}^Nq_i(x,u_i)v_i(u_i)\geq 0\label{eq:beta SOS 1}
\end{align}
\end{subequations}
then $\beta^k$ satisfies Eqn. \eqref{eq:beta}. Furthermore the obtained $\beta^k=\hat{\beta}^k$.
\end{lemma}
\begin{proof}
Let $\beta^k$ be the solution to SOS program \eqref{eq:beta SOS}. Since $p(x)$ and $q(x,u_i)$ are SOS polynomials, we have that $p(x)h(x)\geq 0$ for all $x\in\mathcal{C}_k$ and $q_i(x,u_i)v_i(u_i)\geq 0$ for all $u_i\in\mathcal{U}_i$. Thus $\beta^k$ satisfies that
\begin{multline*}
    \beta^k\leq \sum_{i=m+1}^N\frac{\partial h^k}{\partial x_i}(f_{i,coupled}(x_i,x_{-i})\\
    +g_{i,coupled}(x_i,x_{-i})u_i),~\forall x\in\mathcal{C}_k,u_i\in\mathcal{U}_i,\forall i
\end{multline*}
We can show that $\beta^k=\hat{\beta}^k$ using arguments similar to the proof of Lemma \ref{lemma:1}.
%Assume that there exists some $|\hat{\beta}^k|>|\beta^k|$ such that $\hat{\beta}^k$ satisfies Eqn. \eqref{eq:beta}. Then $\hat{\beta}^k$ is also feasible to constraint \eqref{eq:beta SOS 1}. However, this contradicts the optimality of $\beta^k$ to SOS program \eqref{eq:beta SOS}.
\end{proof}

Now we present our algorithm for computing control policies given the parameters $\gamma_i^k$ and $\beta^k$. To do so, we translate the condition given in \eqref{eq:MR} as SOS constraints and formulate an SOS program to compute the control input $u_i$ for each $i=1, \ldots, N$. The following Lemma presents the result.

\begin{lemma}
Suppose $\gamma_i^k$ and $\beta^k$ are given for each $i\in\{m+1,\ldots,N\}$ and $k\in\{1,\ldots,K\}$. Suppose the following expression are SOS for for each $i\in\{1,\ldots,m\}$ and $k\in\{1,\ldots,K\}$.
\begin{align}
    &\frac{\partial h^k}{\partial x_i}[f_{i,self}(x_i)+g_{i,self}(x_i)\mu_i(x) + f_{i,coupled}(x_i,x_{-i})\nonumber \\
    & \quad +g_{i,coupled}(x_i,x_{-i})\mu_i(x)] - \alpha_i^k\Big(-\eta_i^k(h^k(x))-\beta^k \nonumber \\
    & \quad \quad -\sum_{j=m+1}^N\gamma_j^k\Big) -\sum_{j=1}^K\lambda_i(x)h^j(x), \label{eq:feasibility SOS}
\end{align}
where $\lambda_i(x)$ is an SOS polynomial and $\mu_i(x)$ is a polynomial in $x$.
Then condition \eqref{eq:MR} is satisfied for $x\in\mathcal{C}$ when $u_i$ is chosen as $u_i=\mu_i(x)$.
\end{lemma}
\begin{proof}
Since $\lambda_i(x)$ is an SOS polynomial, we have that $\lambda_i(x)h_k(x)\geq 0$ for all $x\in\mathcal{C}$ implying $\sum_{j=1}^K\lambda_i(x)h^j(x) \geq 0$. When Eqn. \eqref{eq:feasibility SOS} is an SOS, we thus have that 
\begin{align}
    & \frac{\partial h_k}{\partial x_i}[f_{i,self}(x_i)+g_{i,self}(x_i)\mu_i(x) + f_{i,coupled}(x_i,x_{-i}) \nonumber \\
    & \quad +g_{i,coupled}(x_i,x_{-i})\mu_i(x)] - \alpha_i^k\left(-\eta_i^k(h^k(x)) \nonumber \\
    &\quad-\beta^k-\sum_{j=m+1}^N\gamma_j^k\right)\geq 0
\end{align}
holds for all $x\in \mathcal{C}$. By choosing $u_i=\mu_i(x)$, we recover the condition \eqref{eq:MR}.
\end{proof}

Now we present  Algorithm \ref{algo:C1} that uses the above results to find the control policies in the protected sub-systems. First the parameters $\gamma_i^k$ and $\beta^k$ are calculated for each of the vulnerable subsystems and safety constraints. Then using these computed values control input $u_i$ for each $i \in \mathcal{N}_1$ is calculated separately.
If the SOS conditions in \eqref{eq:feasibility SOS} is feasible for all $i \in \mathcal{N}_1$ and $k \in \{1, \ldots K\}$, the algorithm returns the control inputs for all the protected sub-systems. We remark that Algorithm \ref{algo:C1} can be implemented in an offline manner and it calculates control input $u_i$ for each protected sub-system separately.

\begin{center}
  	\begin{algorithm}[!htp]
  		\caption{Solution algorithm for finding control policy}
  		\label{algo:C1}
  		\begin{algorithmic}[1]
  			\State \textbf{Input}: Dynamics $F$. Functions $h_k$ and $v_i$. Constants $\{\alpha_i^k\}$.
  			\State \textbf{Output:} Parameters $\{\gamma_i^k\}_{i=m+1}^N$, $\beta^k$, and $u_i$
            \State Solve the SOS programs in Eqn. \eqref{eq:gamma SOS} and \eqref{eq:beta SOS} to calculate $\gamma_i^k$ and $\beta^k$ for each for each $i\in\{m+1,\ldots,N\}$ and $k\in\{1,\ldots,K\}$.
            \State \textbf{Initialization:} $i \leftarrow 1$, $Flag \leftarrow 1$.
            \While{$Flag=1$ and $i\leq m$}
            \State Solve \eqref{eq:feasibility SOS} using $\gamma_i^k$ and $\beta^k$ for all $k=1, \ldots K$. \label{linecheck}
            \If{Line \ref{linecheck} is feasible}
            \State $u_i=\mu_i$. $i \leftarrow i+1$
            \Else 
            \State $Flag \leftarrow 0$.
            \EndIf
            \EndWhile
            \If{$Flag=1$}
            \State \textbf{return} $\{\gamma_i^k\}$, $\{\beta^k\}$ and $\{u_i\}$
            \Else 
            \State Not feasible.
            \EndIf
  		\end{algorithmic}
  	\end{algorithm}
  \end{center}
  
It may be possible that there exists no control policy that maintain safety of the system depending on the value of $m$ relative to $N$ or the ranges of $\mathcal{U}$ and $\mathcal{C}$ or the model dynamics $F(x,u)$. In that case Algorithm \ref{algo:C1} will fail rendering infeasibility. However, it may happen that Algorithm \ref{algo:C1} is infeasible for $\mathcal{C}$ but feasible for some set $\tilde{\mathcal{C}} \subset \mathcal{C}$. In that case one need to modify the algorithm and search for the set $\tilde{\mathcal{C}}$ such that the algorithm becomes feasible. In that case the system $\mathcal{S}$ will maintain safety for all $t\geq 0$ if $x(0) \in \tilde{\mathcal{C}}$.

It is worthwhile to discuss the case where any of the safety constraints is local to a sub-system. Suppose the safety constraint $h^k(x)$ is local to the sub-system $\mathcal{S}_i$ in the sense that it can be written as $h^k(x_i)$. This implies $\frac{\partial h^k}{\partial x_j}=0$ for $j\neq i$. If $i \in \mathcal{N}_1$, then we have $\sum_{j=m+1}^N\gamma_j^k = \beta^k= 0$. This implies $(m-1)$ conditions in Theorem \ref{Th1} are trivially satisfied and can be omitted from the SOS program. However, if $i \in \mathcal{N}_2$, then our approach can be modified to obtain less conservative SOS formulation. In this case, instead of calculating $\gamma_i^k$ (note, $\gamma_j^k = 0$ for $j\neq i$) and $\beta^k$, we can impose the following constraint directly in each of the SOS program: $\frac{\partial h^k}{\partial x_i}F_i(x_i, x_{-i},u_i) \geq -\eta_i^k( h^k(x_i))$ for all $x\in \mathcal{C}$ and $u_i \in \mathcal{U}_i$. This condition is less conservative than the constraint $\gamma_i^k + \beta^k \geq -\eta_i^k( h^k(x_i))$ obtained via Theorem 1. We remark that $\frac{\partial h^k}{\partial x_i}F_i(x_i, x_{-i},u_i) \geq -\eta_i^k( h^k(x_i))$ introduces infeasibility if the impact of compromised $u_i \in \mathcal{U}_i$ on $h^k(x_i)$ cannot be compensated by the system states.

Now we present two special cases where these parameters or/and the control policies of protected sub-system can be obtained more efficiently relative to SOS approach.

\subsubsection{LTI System with Half-Plane Constraint}
Consider system $\mathcal{S}$ be given as
\begin{equation}
    \mathcal{S}:\dot{x} = Ax+Bu,
\end{equation}
where 
\begin{equation*}
    A=\begin{bmatrix}
    A_{11}&\ldots&A_{1N}\\
    \vdots&\ddots&\vdots\\
    A_{N1}&\ldots&A_{NN}
    \end{bmatrix},\quad B=\begin{bmatrix}
    B_{11}&\ldots&\mathbf{0}\\
    \vdots&\ddots&\vdots\\
    \mathbf{0}&\ldots&B_{NN}
    \end{bmatrix}
\end{equation*}
$A_{ij}\in\mathbb{R}^{n_i\times n_j}$, and $B_{ii}\in\mathbb{R}^{n_i\times r_i}$. 

We consider $h^k(x)=a_k^\top x$ where $a_k\in\mathbb{R}^{n}$ for all $k=1,\ldots,K$. We show that $\gamma_i^k$ can be computed using a linear program when $\mathcal{U}_i=\{u_i:w^\top u_i\geq 0\}$.

For each sub-system $i\in\mathcal{N}_2$, if $\gamma_i^k=a_k^\top(f_{i,self}(x_i^*)+g_{i,self}(x_i^*)u_i^*)$, where $[x_i^*,u_i^*]$ is the solution to the following linear program:
\begin{subequations}\label{eq:gamma LP}
\begin{align}
    \min_{x_i,u_i}~ &a_k^\top(f_{i,self}(x_i)+g_{i,self}(x_i)u_i)\\
    \st ~&a_k^\top x\geq 0,~\forall k\label{eq:gamma LP 1}\\
    &w^\top u_i\geq 0
\end{align}
\end{subequations}
then $\gamma_i^k$ satisfies Eqn. \eqref{eq:gamma}. The statement can be derived by showing that $\gamma_i^k$ attained at the optimal solution of linear program \eqref{eq:gamma LP} satisfies that
\begin{align*}
    \gamma_i^k= a_k^\top(f_{i,self}(x_i^*)+g_{i,self}(x_i^*)u_i^*)
    \leq a_k^\top(f_{i,self}(x_i) \nonumber \\
    +g_{i,self}(x_i)u_i),
\end{align*}
for all $x_i\in \mathcal{C}$ and $u_i\in\mathcal{U}_i$, which satisfies the definition given in Eqn. \eqref{eq:gamma}.

Let $\mathcal{P}$ be the polyhedron induced by the constraints in Eqn. \eqref{eq:gamma LP}. We have that $\gamma_i^k$ is attained at some vertex of $\mathcal{P}$. We then consider the computation of $\beta^k$. For each sub-system $i\in\{m+1,\ldots,N\}$, if $\beta^k=\sum_{i=m+1}^Na_k^\top(f_{i,coupled}(x_i^*,x_{-i}^*)+g_{i,coupled}(x_i^*,x_{-i}^*)u_i^*)$, where $[x^*,u_i^*]$ is the solution to the following linear program:
\begin{subequations}\label{eq:beta LP}
\begin{align}
    \min_{x,u_i}~ &\sum_{i=m+1}^Na_k^\top(f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i)\\
    \st ~&a_k^\top x\geq 0,~\forall k\label{eq:beta LP 1}\\
    &w^\top u_i\geq 0
\end{align}
\end{subequations}
then $\beta^k$ satisfies Eqn. \eqref{eq:beta}.
This statement holds by observing that $\beta^k$ attained at the optimal solution of Eqn. \eqref{eq:beta LP} satisfies that
\begin{multline*}
    \beta^k= \sum_{i=m+1}^Na_k^\top(f_{i,coupled}(x_i^*,x_{-i}^*)+g_{i,coupled}(x_i^*,x_{-i}^*)u_i^*)\\
    \leq\sum_{i=m+1}^Na_k^\top(f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i),
\end{multline*}
for all $x_i\in\cap_{k=1}^K\mathcal{C}_k$ and $u_i\in\mathcal{U}_i$, which satisfies the definition given in Eqn. \eqref{eq:beta}.


\subsubsection{Monotone System with Hyperrectangle Constraints}
In this subsection, we consider monotone systems under hyperrectangle constraints. Consider system \eqref{eq:joint dynamics} and a safety set $\mathcal{C}=[\underline{x},\overline{x}]$, where $\underline{x},\overline{x}\in\mathbb{R}^n$. We consider $\underline{x}\leq \overline{x}$ element-wise, and thus $\mathcal{C}$ is a hyperrectangle. We additionally suppose that $\mathcal{U}_i=[\underline{u}_i,\overline{u}_i]$ is a hyperrectangle.
\begin{definition}[Monotonicity]\label{def:monotone}
Consider system \eqref{eq:joint dynamics}. We say system \eqref{eq:joint dynamics} is monotone with respect to $x$ and $u$ if
\begin{equation}
    x\leq x' \text{ and } u\leq u'\implies F(x,u)\leq F(x',u')
\end{equation}
where the order relation $\leq$ is compared element-wise.
\end{definition}

Using Definition \ref{def:monotone}, Eqn. \eqref{eq:gamma} and \eqref{eq:beta}, we have the following result.
\begin{lemma}
Consider system \eqref{eq:joint dynamics} and a hyperrectangle safety set $\mathcal{C}=[\underline{x},\overline{x}]$. If $F_{ii}(x_i,u_i)=f_{i,self}(x_i)+g_{i,self}(x_i)u_i$ and $F_{i}(x_i,u_i)=f_{i,coupled}(x_i,x_{-i})+g_{i,coupled}(x_i,x_{-i})u_i$ are monotone as given in Definition \ref{def:monotone}, then 
\begin{equation*}
    \gamma_i^k=\frac{\partial h_k}{\partial x_i}(f_{i,self}(\hat{x}_i)+g_{i,self}(\hat{x}_i)\hat{u}_i)
\end{equation*}
where the $z$-th entry of $\hat{x}_i$ is given as
\begin{equation*}
    [\hat{x}_i]_z=\begin{cases}
    [\underline{x}_i]_z\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z\geq 0\\
    [\overline{x}_i]_z\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z< 0
    \end{cases}
\end{equation*}
and $\hat{u}_i$ is given as
\begin{equation*}
    \hat{u}_i=\begin{cases}
    \underline{u}_i\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z\geq 0\\
    \overline{u}_i\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z< 0
    \end{cases}.
\end{equation*}
Moreover, we have that
\begin{equation}
    \beta^k=\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{i,coupled}(\hat{x}_i,\hat{x}_{-i})+g_{i,coupled}(\hat{x}_i,\hat{x}_{-i})\hat{u}_i).
\end{equation}
\end{lemma}

==> solution.tex <==
\section{Solution Approach}\label{sec:sol}

We partition the set of sub-systems $\mathcal{N}=\{1,\ldots,N\}$ as $\{1,\ldots,m\}$ and $\{m+1,\ldots,N\}$. Consider the set of sub-systems that fail or are compromised by the adversary, denoted as $\{m+1,\ldots,N\}$. We first define $\gamma_i^k\in\mathbb{R}$ for each $i=m+1,\ldots,m$ and $k=1,\ldots,K$ as 
\begin{equation}\label{eq:gamma}
    \gamma_i^k = \inf_{x\in\mathcal{C},u_i\in\mathcal{U}_i}\left\{\frac{\partial h}{\partial x_i}(f_{ii}(x_i)+g_{ii}(x_i)u_i)\right\}.
\end{equation}
Variable $\gamma_i^k$ models the contribution from sub-system $i$ towards satisfying/violating the safety constraint of $\mathcal{C}_k$ defined over the joint system when the interconnection among sub-systems is absent. When $\gamma_i^k\geq 0$, it indicates that sub-system $i$ does not cause the safety violation for any $u_i\in\mathcal{U}_i$, provided that there is no interconnection among the sub-systems. We further define
\begin{multline}\label{eq:beta}
    \beta^k=\inf_{x\in\mathcal{C},\prod_{i=m+1}^Nu_i\in\prod_{i=m+1}^N\mathcal{U}_i}\Big\{\sum_{i=m+1}^N\frac{\partial h}{\partial x_i}(f_{i}(x_i,x_{-i})\\
    +g_{i}(x_i,x_{-i})u_i)\Big\}
\end{multline}
Variable $\beta^k$ captures the worst-case impact towards safety violation caused by the interconnection with sub-systems in $\{m+1,\ldots N\}$. When $\beta^k\geq 0$, it indicates the interconnection does not lead to the safety violation for any $\prod_{i=m+1}^Nu_i\in\prod_{i=m+1}^N\mathcal{U}_i$.

In the following, we present how to calculate $\gamma_i^k$ and $\beta^k$. We make the following assumption.
\begin{assumption}\label{assump:semi-algebraic}
We assume that $h_k(x)$ is polynomial in $x$ and $\mathcal{U}_i=\{u_i:v(u_i)\geq 0\}$ for each $k=1,\ldots,K$, where $v$ is polynomial in $u_i$ for all $i\in\{m+1,\ldots,N\}$.
\end{assumption}
For each $i=m+1,\ldots,N$, we use the following result to compute $\gamma_i^k$ for each $i\in\{m+1,\ldots,N\}$.
\begin{lemma}
Suppose Assumption \ref{assump:semi-algebraic} holds. For each sub-system $i\in\{m+1,\ldots,N\}$, if there exist sum-of-squares polynomials $p(x)$ and $q(x,u_i)$ such that $\gamma_i^k$ is the solution to the following sum-of-squares program:
\begin{subequations}\label{eq:gamma SOS}
\begin{align}
    \min_{\gamma_i^k}~ &-\gamma_i^k\\
    \st ~&\frac{\partial h_k}{\partial x_i}(f_{ii}(x_i)+g_{ii}(x_i)u_i)\nonumber\\
    &\quad\quad\quad-\gamma_i-p(x)h_k(x)-q(x,u_i)v(u_i)\geq 0\label{eq:gamma SOS 1}
\end{align}
\end{subequations}
then $\gamma_i^k$ satisfies Eqn. \eqref{eq:gamma}.
\end{lemma}
\begin{proof}
Let $\gamma_i^k$ be the solution to SOS program \eqref{eq:gamma SOS}. Since $p(x)$ and $q(x,u_i)$ are SOS polynomials, we have that $p(x)h_k(x)\geq 0$ for all $x\in\mathcal{C}_k$ and $q(x,u_i)v(u_i)\geq 0$ for all $u_i\in\mathcal{U}_i$. Thus $\gamma_i^k$ satisfies that
\begin{equation*}
    \gamma_i^k\leq \frac{\partial h_k}{\partial x_i}(f_{ii}(x_i)+g_{ii}(x_i)u_i),~\forall x\in\mathcal{C}_k,u_i\in\mathcal{U}_i
\end{equation*}
Assume that there exists some $|\hat{\gamma}_i^k|>|\gamma_i^k|$ such that $\hat{\gamma}_i^k$ satisfies Eqn. \eqref{eq:gamma}. Then $\hat{\gamma}_i^k$ is also feasible to constraint \eqref{eq:gamma SOS 1}. However, this contradicts the optimality of $\gamma_i$ to SOS program \eqref{eq:gamma SOS}.
\end{proof}

We solve for $\beta^k$ using the following lemma.
\begin{lemma}
Suppose Assumption \ref{assump:semi-algebraic} holds. If there exist sum-of-squares polynomials $p(x)$ and $q_i(x,u_i)$ such that $\beta^k$ is the solution to the following sum-of-squares program:
\begin{subequations}\label{eq:beta SOS}
\begin{align}
    \min_{\beta^k}~ &-\beta^k\\
    \st ~&\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})u_i)\nonumber\\
    &\quad-\beta-p(x)h_k(x)-\sum_{i=m+1}^Nq_i(x,u_i)v_i(u_i)\geq 0\label{eq:beta SOS 1}
\end{align}
\end{subequations}
then $\beta^k$ satisfies Eqn. \eqref{eq:beta}.
\end{lemma}
\begin{proof}
Let $\beta^k$ be the solution to SOS program \eqref{eq:beta SOS}. Since $p(x)$ and $q(x,u_i)$ are SOS polynomials, we have that $p(x)h(x)\geq 0$ for all $x\in\mathcal{C}_k$ and $q_i(x,u_i)v_i(u_i)\geq 0$ for all $u_i\in\mathcal{U}_i$. Thus $\beta^k$ satisfies that
\begin{equation*}
    \beta^k\leq \sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{i}(x_i,x_{-i})\\
    +g_{i}(x_i,x_{-i})u_i),~\forall x\in\mathcal{C}_k,u_i\in\mathcal{U}_i,\forall i
\end{equation*}
Assume that there exists some $|\hat{\beta}^k|>|\beta^k|$ such that $\hat{\beta}^k$ satisfies Eqn. \eqref{eq:beta}. Then $\hat{\beta}^k$ is also feasible to constraint \eqref{eq:beta SOS 1}. However, this contradicts the optimality of $\beta^k$ to SOS program \eqref{eq:beta SOS}.
\end{proof}

Given the values of $\gamma_i^k$ and $\beta^k$, we can then compute the control input $u_i$ for each $i\in\{1,\ldots,m\}$ as follows:
\begin{subequations}\label{eq:QP}
\begin{align}
    \min_{u_i}~&u_i^\top u_i\\
    \st ~& \frac{\partial h_k}{\partial x_i}[f_{ii}(x_i)+g_{ii}(x_i)u_i + f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})u_i]\nonumber\\
    &\quad\geq \alpha_i\left(-\eta_i(h_k(x))-\beta^k-\sum_{j=m+1}^N\gamma_j^k\right),~\forall k\label{eq:QP 1}
\end{align}
\end{subequations}
where $\alpha_i\in[0,1]$ is a constant satisfying $\sum_{i=1}^m\alpha_i=1$ and $\eta_i:\mathbb{R}^n\rightarrow\mathbb{R}$ is an extended class $\mathcal{K}$ function. We prove the safety guarantee provided by the solution of Eqn. \eqref{eq:QP} as follows:
\begin{theorem}
Let $u_i$ be computed by solving Eqn. \eqref{eq:QP} at each time $t$ for sub-systems $i\in\{1,\ldots,m\}$. We have that $x\in\mathcal{C}_k$ for system $\mathcal{S}$ by implementing $u_i$ for each sub-system $i\in \{1,\ldots,m\}$, provided that the initial state is in $\mathcal{C}_k$.
\end{theorem}
\begin{proof}
Let $F(x,u)$ be the dynamics of system $\mathcal{S}$. We compute $\frac{\partial h_k}{\partial x}F(x,u)$ for each $k=1,\ldots,K$ as
\begin{align}
    &\frac{\partial h_k}{\partial x}F(x,u)\nonumber\\
    =&\sum_{i=1}^N\frac{\partial h_k}{\partial x_i}F_i(x_i,x_{-i},u_i)\\
    =&\sum_{i=1}^m\frac{\partial h_k}{\partial x_i}F_i(x_i,x_{-i},u_i)+\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}F_i(x_i,x_{-i},u_i)\\
    =&\sum_{i=1}^m\frac{\partial h_k}{\partial x_i}[f_{ii}(x_i)+f_i(x_i,x_{-i})+g_{ii}(x_i)+g_{i}(x_i,x_{-i})u_i] \nonumber\\
    &+ \sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}[f_{ii}(x_i)+f_i(x_i,x_{-i})+g_{ii}(x_i)+g_{i}(x_i,x_{-i})u_i]\\
    \geq &-\sum_{i=1}^m\alpha_i \eta_i(h_k(x))-\beta^k-\sum_{j=m+1}^N\gamma_j^k\nonumber\\
    &\quad\quad+\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{ii}(x_i)+g_{ii}(x_i)u_i)\nonumber\\
    &\quad\quad+\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{i}(x_i,x_{-i})
    +g_{i}(x_i,x_{-i})u_i)\\
    \geq &-\sum_{i=1}^m\alpha_i \eta_i(h_k(x))
\end{align}
where the first inequality holds by the fact that $u_i$ is the solution of Eqn. \eqref{eq:QP} and the last inequality holds by the definitions of $\gamma_i^k$ and $\beta^k$. Since that $\eta_i$ is an extended class $\mathcal{K}$ function and $\alpha_i\in[0,1]$, we have that $\sum_{i}\alpha_i\eta_i$ is also an extended class $K$ function. Thus $\frac{\partial h_k}{\partial x}F(x,u)\geq -\eta(h_k(x))$. Using \cite{ames2016control}, we have that system $\mathcal{S}$ is safe with respect to $\mathcal{C}_k$ for all $k=1,\ldots,K$.
\end{proof}

Note that the optimization problem in Eqn. \eqref{eq:QP} is a quadratic program and can be solved efficiently using the existing solvers in real time. However, the existence of $u_i$ relies on the choice of $\alpha_i$ and the assumption that constraint \eqref{eq:QP 1} is feasible for all $x\in\mathcal{C}$, which may not be true for any system. To eliminate the dependence on $\alpha_i$, we can set $\alpha_i$ as an additional decision variable in Eqn. \eqref{eq:QP} and add a constraint $\sum_{i=1}^m\alpha_i=1$, without impairing its convexity. In the next section, we present an offline verification process to relax the assumption on the feasibility of constraint \eqref{eq:QP 1}.

==> special_case.tex <==
\section{Special Case}

In this section, we present some special cases to compute parameters $\gamma_i^k$ and $\beta^k$ more efficiently compared with the SOS programs in Eqn. \eqref{eq:gamma SOS} and \eqref{eq:beta SOS}.

\subsection{LTI System with Half-Plane Constraint}
Consider system $\mathcal{S}$ be given as
\begin{equation}
    \mathcal{S}:\dot{x} = Ax+Bu,
\end{equation}
where 
\begin{equation*}
    A=\begin{bmatrix}
    A_{11}&\ldots&A_{1N}\\
    \vdots&\ddots&\vdots\\
    A_{N1}&\ldots&A_{NN}
    \end{bmatrix},\quad B=\begin{bmatrix}
    B_{11}&\ldots&\mathbf{0}\\
    \vdots&\ddots&\vdots\\
    \mathbf{0}&\ldots&B_{NN}
    \end{bmatrix}
\end{equation*}
$A_{ij}\in\mathbb{R}^{n_i\times n_j}$, and $B_{ii}\in\mathbb{R}^{n_i\times r_i}$. 

We consider $h_k(x)=a_k^\top x$ where $a_k\in\mathbb{R}^{n}$ for all $k=1,\ldots,K$. We show that $\gamma_i^k$ can be computed using a linear program when $\mathcal{U}_i=\{u_i:w^\top u_i\geq 0\}$.
\begin{lemma}
For each sub-system $i\in\{m+1,\ldots,N\}$, if $\gamma_i^k=a_k^\top(f_{ii}(x_i^*)+g_{ii}(x_i^*)u_i^*)$, where $[x_i^*,u_i^*]$ is the solution to the following linear program:
\begin{subequations}\label{eq:gamma LP}
\begin{align}
    \min_{x_i,u_i}~ &a_k^\top(f_{ii}(x_i)+g_{ii}(x_i)u_i)\\
    \st ~&a_k^\top x\geq 0,~\forall k\label{eq:gamma LP 1}\\
    &w^\top u_i\geq 0
\end{align}
\end{subequations}
then $\gamma_i^k$ satisfies Eqn. \eqref{eq:gamma}.
\end{lemma}
\begin{proof}
Let $\gamma_i^k$ be the solution to linear program \eqref{eq:gamma LP}. Thus $\gamma_i^k$ satisfies that
\begin{equation*}
    \gamma_i^k= a_k^\top(f_{ii}(x_i^*)+g_{ii}(x_i^*)u_i^*)
    \leq a_k^\top(f_{ii}(x_i)+g_{ii}(x_i)u_i),
\end{equation*}
for all $x_i\in\cap_{k=1}^K\mathcal{C}_k$ and $u_i\in\mathcal{U}_i$, which satisfies the definition given in Eqn. \eqref{eq:gamma}.
\end{proof}
Let $\mathcal{P}$ be the polyhedron induced by the constraints in Eqn. \eqref{eq:gamma LP}. We have that $\gamma_i^k$ is attained at some vertex of $\mathcal{P}$. Similarly, parameter $\beta^k$ can be obtained using the following result.
\begin{lemma}
For each sub-system $i\in\{m+1,\ldots,N\}$, if $\beta^k=\sum_{i=m+1}^Na_k^\top(f_{i}(x_i^*,x_{-i}^*)+g_{i}(x_i^*,x_{-i}^*)u_i^*)$, where $[x^*,u_i^*]$ is the solution to the following linear program:
\begin{subequations}\label{eq:beta LP}
\begin{align}
    \min_{x,u_i}~ &\sum_{i=m+1}^Na_k^\top(f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})u_i)\\
    \st ~&a_k^\top x\geq 0,~\forall k\label{eq:beta LP 1}\\
    &w^\top u_i\geq 0
\end{align}
\end{subequations}
then $\beta^k$ satisfies Eqn. \eqref{eq:beta}.
\end{lemma}
\begin{proof}
Let $\beta^k$ be the solution to linear program \eqref{eq:beta LP}. Thus $\beta^k$ satisfies that
\begin{multline*}
    \beta^k= \sum_{i=m+1}^Na_k^\top(f_{i}(x_i^*,x_{-i}^*)+g_{i}(x_i^*,x_{-i}^*)u_i^*)\\
    \leq\sum_{i=m+1}^Na_k^\top(f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})u_i),
\end{multline*}
for all $x_i\in\cap_{k=1}^K\mathcal{C}_k$ and $u_i\in\mathcal{U}_i$, which satisfies the definition given in Eqn. \eqref{eq:beta}.
\end{proof}

\subsection{Monotone System with Hyperrectangle Constraints}
In this subsection, we consider monotone systems under hyperrectangle constraints. Consider system \eqref{eq:joint dynamics} and a safety set $\mathcal{C}=[\underline{x},\overline{x}]$, where $\underline{x},\overline{x}\in\mathbb{R}^n$. We consider $\underline{x}\leq \overline{x}$ element-wise, and thus $\mathcal{C}$ is a hyperrectangle. We additionally suppose that $\mathcal{U}_i=[\underline{u}_i,\overline{u}_i]$ is a hyperrectangle.
\begin{definition}[Monotonicity]\label{def:monotone}
Consider system \eqref{eq:joint dynamics}. We say system \eqref{eq:joint dynamics} is monotone with respect to $x$ and $u$ if
\begin{equation}
    x\leq x' \text{ and } u\leq u'\implies F(x,u)\leq F(x',u')
\end{equation}
where the order relation $\leq$ is compared element-wise.
\end{definition}

Using Definition \ref{def:monotone}, Eqn. \eqref{eq:gamma} and \eqref{eq:beta}, we have the following result.
\begin{corollary}
Consider system \eqref{eq:joint dynamics} and a hyperrectangle safety set $\mathcal{C}=[\underline{x},\overline{x}]$. If $F_{ii}(x_i,u_i)=f_{ii}(x_i)+g_{ii}(x_i)u_i$ and $F_{i}(x_i,u_i)=f_{i}(x_i,x_{-i})+g_{i}(x_i,x_{-i})u_i$ are monotone as given in Definition \ref{def:monotone}, then 
\begin{equation*}
    \gamma_i^k=\frac{\partial h_k}{\partial x_i}(f_{ii}(\hat{x}_i)+g_{ii}(\hat{x}_i)\hat{u}_i)
\end{equation*}
where the $z$-th entry of $\hat{x}_i$ is given as
\begin{equation*}
    [\hat{x}_i]_z=\begin{cases}
    [\underline{x}_i]_z\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z\geq 0\\
    [\overline{x}_i]_z\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z< 0
    \end{cases}
\end{equation*}
and $\hat{u}_i$ is given as
\begin{equation*}
    \hat{u}_i=\begin{cases}
    \underline{u}_i\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z\geq 0\\
    \overline{u}_i\mbox{ if }[\frac{\partial h_k}{\partial x_i}]_z< 0
    \end{cases}.
\end{equation*}
Moreover, we have that
\begin{equation}
    \beta^k=\sum_{i=m+1}^N\frac{\partial h_k}{\partial x_i}(f_{i}(\hat{x}_i,\hat{x}_{-i})+g_{i}(\hat{x}_i,\hat{x}_{-i})\hat{u}_i).
\end{equation}
\end{corollary}
